Observation of $B^0_s$-$\bar{B}^0_s$ mixing and measurement of mixing frequencies using semileptonic B decays

The $B^0_s$ and $B^0$ mixing frequencies, $\Delta m_s$ and $\Delta m_d$, are measured using a data sample corresponding to an integrated luminosity of 1.0 fb^{-1} collected by the LHCb experiment in $pp$ collisions at a centre of mass energy of 7 TeV during 2011. Around 1.8x10^6 candidate events are selected of the type $B^0_{(s)} \to D^-_{(s)} \mu^+$ (+ anything), where about half are from peaking and combinatorial backgrounds. To determine the B decay times, a correction is required for the momentum carried by missing particles, which is performed using a simulation-based statistical method. Associated production of muons or mesons allows us to tag the initial-state flavour and so to resolve oscillations due to mixing. We obtain \Delta m_s = (17.93 \pm 0.22 (stat) \pm 0.15 (syst)) ps^{-1}, \Delta m_d = (0.503 \pm 0.011 (stat) \pm 0.013 (syst)) ps^{-1}. The hypothesis of no oscillations is rejected by the equivalent of 5.8 standard deviations for $B^0_s$ and 13.0 standard deviations for $B^0$. This is the first observation of $B^0_s$ mixing to be made using only semileptonic decays.

==> Authors/LHCb_HD_authorlist_2013-06-18_previous.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
R.~Aaij$^{40}$, 
B.~Adeva$^{36}$, 
M.~Adinolfi$^{45}$, 
C.~Adrover$^{6}$, 
A.~Affolder$^{51}$, 
Z.~Ajaltouni$^{5}$, 
J.~Albrecht$^{9}$, 
F.~Alessio$^{37}$, 
M.~Alexander$^{50}$, 
S.~Ali$^{40}$, 
G.~Alkhazov$^{29}$, 
P.~Alvarez~Cartelle$^{36}$, 
A.A.~Alves~Jr$^{24,37}$, 
S.~Amato$^{2}$, 
S.~Amerio$^{21}$, 
Y.~Amhis$^{7}$, 
L.~Anderlini$^{17,f}$, 
J.~Anderson$^{39}$, 
R.~Andreassen$^{56}$, 
J.E.~Andrews$^{57}$, 
R.B.~Appleby$^{53}$, 
O.~Aquines~Gutierrez$^{10}$, 
F.~Archilli$^{18}$, 
A.~Artamonov$^{34}$, 
M.~Artuso$^{58}$, 
E.~Aslanides$^{6}$, 
G.~Auriemma$^{24,m}$, 
M.~Baalouch$^{5}$, 
S.~Bachmann$^{11}$, 
J.J.~Back$^{47}$, 
C.~Baesso$^{59}$, 
V.~Balagura$^{30}$, 
W.~Baldini$^{16}$, 
R.J.~Barlow$^{53}$, 
C.~Barschel$^{37}$, 
S.~Barsuk$^{7}$, 
W.~Barter$^{46}$, 
Th.~Bauer$^{40}$, 
A.~Bay$^{38}$, 
J.~Beddow$^{50}$, 
F.~Bedeschi$^{22}$, 
I.~Bediaga$^{1}$, 
S.~Belogurov$^{30}$, 
K.~Belous$^{34}$, 
I.~Belyaev$^{30}$, 
E.~Ben-Haim$^{8}$, 
G.~Bencivenni$^{18}$, 
S.~Benson$^{49}$, 
J.~Benton$^{45}$, 
A.~Berezhnoy$^{31}$, 
R.~Bernet$^{39}$, 
M.-O.~Bettler$^{46}$, 
M.~van~Beuzekom$^{40}$, 
A.~Bien$^{11}$, 
S.~Bifani$^{44}$, 
T.~Bird$^{53}$, 
A.~Bizzeti$^{17,h}$, 
P.M.~Bj\o rnstad$^{53}$, 
T.~Blake$^{37}$, 
F.~Blanc$^{38}$, 
J.~Blouw$^{11}$, 
S.~Blusk$^{58}$, 
V.~Bocci$^{24}$, 
A.~Bondar$^{33}$, 
N.~Bondar$^{29}$, 
W.~Bonivento$^{15}$, 
S.~Borghi$^{53}$, 
A.~Borgia$^{58}$, 
T.J.V.~Bowcock$^{51}$, 
E.~Bowen$^{39}$, 
C.~Bozzi$^{16}$, 
T.~Brambach$^{9}$, 
J.~van~den~Brand$^{41}$, 
J.~Bressieux$^{38}$, 
D.~Brett$^{53}$, 
M.~Britsch$^{10}$, 
T.~Britton$^{58}$, 
N.H.~Brook$^{45}$, 
H.~Brown$^{51}$, 
I.~Burducea$^{28}$, 
A.~Bursche$^{39}$, 
G.~Busetto$^{21,q}$, 
J.~Buytaert$^{37}$, 
S.~Cadeddu$^{15}$, 
O.~Callot$^{7}$, 
M.~Calvi$^{20,j}$, 
M.~Calvo~Gomez$^{35,n}$, 
A.~Camboni$^{35}$, 
P.~Campana$^{18,37}$, 
D.~Campora~Perez$^{37}$, 
A.~Carbone$^{14,c}$, 
G.~Carboni$^{23,k}$, 
R.~Cardinale$^{19,i}$, 
A.~Cardini$^{15}$, 
H.~Carranza-Mejia$^{49}$, 
L.~Carson$^{52}$, 
K.~Carvalho~Akiba$^{2}$, 
G.~Casse$^{51}$, 
L.~Castillo~Garcia$^{37}$, 
M.~Cattaneo$^{37}$, 
Ch.~Cauet$^{9}$, 
R.~Cenci$^{57}$, 
M.~Charles$^{54}$, 
Ph.~Charpentier$^{37}$, 
P.~Chen$^{3,38}$, 
N.~Chiapolini$^{39}$, 
M.~Chrzaszcz$^{25}$, 
K.~Ciba$^{37}$, 
X.~Cid~Vidal$^{37}$, 
G.~Ciezarek$^{52}$, 
P.E.L.~Clarke$^{49}$, 
M.~Clemencic$^{37}$, 
H.V.~Cliff$^{46}$, 
J.~Closier$^{37}$, 
C.~Coca$^{28}$, 
V.~Coco$^{40}$, 
J.~Cogan$^{6}$, 
E.~Cogneras$^{5}$, 
P.~Collins$^{37}$, 
A.~Comerma-Montells$^{35}$, 
A.~Contu$^{15,37}$, 
A.~Cook$^{45}$, 
M.~Coombes$^{45}$, 
S.~Coquereau$^{8}$, 
G.~Corti$^{37}$, 
B.~Couturier$^{37}$, 
G.A.~Cowan$^{49}$, 
D.C.~Craik$^{47}$, 
S.~Cunliffe$^{52}$, 
R.~Currie$^{49}$, 
C.~D'Ambrosio$^{37}$, 
P.~David$^{8}$, 
P.N.Y.~David$^{40}$, 
A.~Davis$^{56}$, 
I.~De~Bonis$^{4}$, 
K.~De~Bruyn$^{40}$, 
S.~De~Capua$^{53}$, 
M.~De~Cian$^{11}$, 
J.M.~De~Miranda$^{1}$, 
L.~De~Paula$^{2}$, 
W.~De~Silva$^{56}$, 
P.~De~Simone$^{18}$, 
D.~Decamp$^{4}$, 
M.~Deckenhoff$^{9}$, 
L.~Del~Buono$^{8}$, 
N.~D\'{e}l\'{e}age$^{4}$, 
D.~Derkach$^{54}$, 
O.~Deschamps$^{5}$, 
F.~Dettori$^{41}$, 
A.~Di~Canto$^{11}$, 
H.~Dijkstra$^{37}$, 
M.~Dogaru$^{28}$, 
S.~Donleavy$^{51}$, 
F.~Dordei$^{11}$, 
A.~Dosil~Su\'{a}rez$^{36}$, 
D.~Dossett$^{47}$, 
A.~Dovbnya$^{42}$, 
F.~Dupertuis$^{38}$, 
P.~Durante$^{37}$, 
R.~Dzhelyadin$^{34}$, 
A.~Dziurda$^{25}$, 
A.~Dzyuba$^{29}$, 
S.~Easo$^{48}$, 
U.~Egede$^{52}$, 
V.~Egorychev$^{30}$, 
S.~Eidelman$^{33}$, 
D.~van~Eijk$^{40}$, 
S.~Eisenhardt$^{49}$, 
U.~Eitschberger$^{9}$, 
R.~Ekelhof$^{9}$, 
L.~Eklund$^{50,37}$, 
I.~El~Rifai$^{5}$, 
Ch.~Elsasser$^{39}$, 
A.~Falabella$^{14,e}$, 
C.~F\"{a}rber$^{11}$, 
G.~Fardell$^{49}$, 
C.~Farinelli$^{40}$, 
S.~Farry$^{51}$, 
D.~Ferguson$^{49}$, 
V.~Fernandez~Albor$^{36}$, 
F.~Ferreira~Rodrigues$^{1}$, 
M.~Ferro-Luzzi$^{37}$, 
S.~Filippov$^{32}$, 
M.~Fiore$^{16}$, 
C.~Fitzpatrick$^{37}$, 
M.~Fontana$^{10}$, 
F.~Fontanelli$^{19,i}$, 
R.~Forty$^{37}$, 
O.~Francisco$^{2}$, 
M.~Frank$^{37}$, 
C.~Frei$^{37}$, 
M.~Frosini$^{17,f}$, 
S.~Furcas$^{20}$, 
E.~Furfaro$^{23,k}$, 
A.~Gallas~Torreira$^{36}$, 
D.~Galli$^{14,c}$, 
M.~Gandelman$^{2}$, 
P.~Gandini$^{58}$, 
Y.~Gao$^{3}$, 
J.~Garofoli$^{58}$, 
P.~Garosi$^{53}$, 
J.~Garra~Tico$^{46}$, 
L.~Garrido$^{35}$, 
C.~Gaspar$^{37}$, 
R.~Gauld$^{54}$, 
E.~Gersabeck$^{11}$, 
M.~Gersabeck$^{53}$, 
T.~Gershon$^{47,37}$, 
Ph.~Ghez$^{4}$, 
V.~Gibson$^{46}$, 
L.~Giubega$^{28}$, 
V.V.~Gligorov$^{37}$, 
C.~G\"{o}bel$^{59}$, 
D.~Golubkov$^{30}$, 
A.~Golutvin$^{52,30,37}$, 
A.~Gomes$^{2}$, 
P.~Gorbounov$^{30,37}$, 
H.~Gordon$^{54}$, 
M.~Grabalosa~G\'{a}ndara$^{5}$, 
R.~Graciani~Diaz$^{35}$, 
L.A.~Granado~Cardoso$^{37}$, 
E.~Graug\'{e}s$^{35}$, 
G.~Graziani$^{17}$, 
A.~Grecu$^{28}$, 
E.~Greening$^{54}$, 
S.~Gregson$^{46}$, 
P.~Griffith$^{44}$, 
O.~Gr\"{u}nberg$^{60}$, 
B.~Gui$^{58}$, 
E.~Gushchin$^{32}$, 
Yu.~Guz$^{34,37}$, 
T.~Gys$^{37}$, 
C.~Hadjivasiliou$^{58}$, 
G.~Haefeli$^{38}$, 
C.~Haen$^{37}$, 
S.C.~Haines$^{46}$, 
S.~Hall$^{52}$, 
B.~Hamilton$^{57}$, 
T.~Hampson$^{45}$, 
S.~Hansmann-Menzemer$^{11}$, 
N.~Harnew$^{54}$, 
S.T.~Harnew$^{45}$, 
J.~Harrison$^{53}$, 
T.~Hartmann$^{60}$, 
J.~He$^{37}$, 
T.~Head$^{37}$, 
V.~Heijne$^{40}$, 
K.~Hennessy$^{51}$, 
P.~Henrard$^{5}$, 
J.A.~Hernando~Morata$^{36}$, 
E.~van~Herwijnen$^{37}$, 
M.~Hess$^{60}$, 
A.~Hicheur$^{1}$, 
E.~Hicks$^{51}$, 
D.~Hill$^{54}$, 
M.~Hoballah$^{5}$, 
C.~Hombach$^{53}$, 
P.~Hopchev$^{4}$, 
W.~Hulsbergen$^{40}$, 
P.~Hunt$^{54}$, 
T.~Huse$^{51}$, 
N.~Hussain$^{54}$, 
D.~Hutchcroft$^{51}$, 
D.~Hynds$^{50}$, 
V.~Iakovenko$^{43}$, 
M.~Idzik$^{26}$, 
P.~Ilten$^{12}$, 
R.~Jacobsson$^{37}$, 
A.~Jaeger$^{11}$, 
E.~Jans$^{40}$, 
P.~Jaton$^{38}$, 
A.~Jawahery$^{57}$, 
F.~Jing$^{3}$, 
M.~John$^{54}$, 
D.~Johnson$^{54}$, 
C.R.~Jones$^{46}$, 
C.~Joram$^{37}$, 
B.~Jost$^{37}$, 
M.~Kaballo$^{9}$, 
S.~Kandybei$^{42}$, 
W.~Kanso$^{6}$, 
M.~Karacson$^{37}$, 
T.M.~Karbach$^{37}$, 
I.R.~Kenyon$^{44}$, 
T.~Ketel$^{41}$, 
A.~Keune$^{38}$, 
B.~Khanji$^{20}$, 
O.~Kochebina$^{7}$, 
I.~Komarov$^{38}$, 
R.F.~Koopman$^{41}$, 
P.~Koppenburg$^{40}$, 
M.~Korolev$^{31}$, 
A.~Kozlinskiy$^{40}$, 
L.~Kravchuk$^{32}$, 
K.~Kreplin$^{11}$, 
M.~Kreps$^{47}$, 
G.~Krocker$^{11}$, 
P.~Krokovny$^{33}$, 
F.~Kruse$^{9}$, 
M.~Kucharczyk$^{20,25,j}$, 
V.~Kudryavtsev$^{33}$, 
K.~Kurek$^{27}$, 
T.~Kvaratskheliya$^{30,37}$, 
V.N.~La~Thi$^{38}$, 
D.~Lacarrere$^{37}$, 
G.~Lafferty$^{53}$, 
A.~Lai$^{15}$, 
D.~Lambert$^{49}$, 
R.W.~Lambert$^{41}$, 
E.~Lanciotti$^{37}$, 
G.~Lanfranchi$^{18}$, 
C.~Langenbruch$^{37}$, 
T.~Latham$^{47}$, 
C.~Lazzeroni$^{44}$, 
R.~Le~Gac$^{6}$, 
J.~van~Leerdam$^{40}$, 
J.-P.~Lees$^{4}$, 
R.~Lef\`{e}vre$^{5}$, 
A.~Leflat$^{31}$, 
J.~Lefran\c{c}ois$^{7}$, 
S.~Leo$^{22}$, 
O.~Leroy$^{6}$, 
T.~Lesiak$^{25}$, 
B.~Leverington$^{11}$, 
Y.~Li$^{3}$, 
L.~Li~Gioi$^{5}$, 
M.~Liles$^{51}$, 
R.~Lindner$^{37}$, 
C.~Linn$^{11}$, 
B.~Liu$^{3}$, 
G.~Liu$^{37}$, 
S.~Lohn$^{37}$, 
I.~Longstaff$^{50}$, 
J.H.~Lopes$^{2}$, 
N.~Lopez-March$^{38}$, 
H.~Lu$^{3}$, 
D.~Lucchesi$^{21,q}$, 
J.~Luisier$^{38}$, 
H.~Luo$^{49}$, 
F.~Machefert$^{7}$, 
I.V.~Machikhiliyan$^{4,30}$, 
F.~Maciuc$^{28}$, 
O.~Maev$^{29,37}$, 
S.~Malde$^{54}$, 
G.~Manca$^{15,d}$, 
G.~Mancinelli$^{6}$, 
J.~Maratas$^{5}$, 
U.~Marconi$^{14}$, 
P.~Marino$^{22,s}$, 
R.~M\"{a}rki$^{38}$, 
J.~Marks$^{11}$, 
G.~Martellotti$^{24}$, 
A.~Martens$^{8}$, 
A.~Mart\'{i}n~S\'{a}nchez$^{7}$, 
M.~Martinelli$^{40}$, 
D.~Martinez~Santos$^{41}$, 
D.~Martins~Tostes$^{2}$, 
A.~Massafferri$^{1}$, 
R.~Matev$^{37}$, 
Z.~Mathe$^{37}$, 
C.~Matteuzzi$^{20}$, 
E.~Maurice$^{6}$, 
A.~Mazurov$^{16,32,37,e}$, 
B.~Mc~Skelly$^{51}$, 
J.~McCarthy$^{44}$, 
A.~McNab$^{53}$, 
R.~McNulty$^{12}$, 
B.~Meadows$^{56,54}$, 
F.~Meier$^{9}$, 
M.~Meissner$^{11}$, 
M.~Merk$^{40}$, 
D.A.~Milanes$^{8}$, 
M.-N.~Minard$^{4}$, 
J.~Molina~Rodriguez$^{59}$, 
S.~Monteil$^{5}$, 
D.~Moran$^{53}$, 
P.~Morawski$^{25}$, 
A.~Mord\`{a}$^{6}$, 
M.J.~Morello$^{22,s}$, 
R.~Mountain$^{58}$, 
I.~Mous$^{40}$, 
F.~Muheim$^{49}$, 
K.~M\"{u}ller$^{39}$, 
R.~Muresan$^{28}$, 
B.~Muryn$^{26}$, 
B.~Muster$^{38}$, 
P.~Naik$^{45}$, 
T.~Nakada$^{38}$, 
R.~Nandakumar$^{48}$, 
I.~Nasteva$^{1}$, 
M.~Needham$^{49}$, 
S.~Neubert$^{37}$, 
N.~Neufeld$^{37}$, 
A.D.~Nguyen$^{38}$, 
T.D.~Nguyen$^{38}$, 
C.~Nguyen-Mau$^{38,o}$, 
M.~Nicol$^{7}$, 
V.~Niess$^{5}$, 
R.~Niet$^{9}$, 
N.~Nikitin$^{31}$, 
T.~Nikodem$^{11}$, 
A.~Nomerotski$^{54}$, 
A.~Novoselov$^{34}$, 
A.~Oblakowska-Mucha$^{26}$, 
V.~Obraztsov$^{34}$, 
S.~Oggero$^{40}$, 
S.~Ogilvy$^{50}$, 
O.~Okhrimenko$^{43}$, 
R.~Oldeman$^{15,d}$, 
M.~Orlandea$^{28}$, 
J.M.~Otalora~Goicochea$^{2}$, 
P.~Owen$^{52}$, 
A.~Oyanguren$^{35}$, 
B.K.~Pal$^{58}$, 
A.~Palano$^{13,b}$, 
T.~Palczewski$^{27}$, 
M.~Palutan$^{18}$, 
J.~Panman$^{37}$, 
A.~Papanestis$^{48}$, 
M.~Pappagallo$^{50}$, 
C.~Parkes$^{53}$, 
C.J.~Parkinson$^{52}$, 
G.~Passaleva$^{17}$, 
G.D.~Patel$^{51}$, 
M.~Patel$^{52}$, 
G.N.~Patrick$^{48}$, 
C.~Patrignani$^{19,i}$, 
C.~Pavel-Nicorescu$^{28}$, 
A.~Pazos~Alvarez$^{36}$, 
A.~Pellegrino$^{40}$, 
G.~Penso$^{24,l}$, 
M.~Pepe~Altarelli$^{37}$, 
S.~Perazzini$^{14,c}$, 
E.~Perez~Trigo$^{36}$, 
A.~P\'{e}rez-Calero~Yzquierdo$^{35}$, 
P.~Perret$^{5}$, 
M.~Perrin-Terrin$^{6}$, 
L.~Pescatore$^{44}$, 
E.~Pesen$^{61}$, 
G.~Pessina$^{20}$, 
K.~Petridis$^{52}$, 
A.~Petrolini$^{19,i}$, 
A.~Phan$^{58}$, 
E.~Picatoste~Olloqui$^{35}$, 
B.~Pietrzyk$^{4}$, 
T.~Pila\v{r}$^{47}$, 
D.~Pinci$^{24}$, 
S.~Playfer$^{49}$, 
M.~Plo~Casasus$^{36}$, 
F.~Polci$^{8}$, 
G.~Polok$^{25}$, 
A.~Poluektov$^{47,33}$, 
E.~Polycarpo$^{2}$, 
A.~Popov$^{34}$, 
D.~Popov$^{10}$, 
B.~Popovici$^{28}$, 
C.~Potterat$^{35}$, 
A.~Powell$^{54}$, 
J.~Prisciandaro$^{38}$, 
A.~Pritchard$^{51}$, 
C.~Prouve$^{7}$, 
V.~Pugatch$^{43}$, 
A.~Puig~Navarro$^{38}$, 
G.~Punzi$^{22,r}$, 
W.~Qian$^{4}$, 
J.H.~Rademacker$^{45}$, 
B.~Rakotomiaramanana$^{38}$, 
M.S.~Rangel$^{2}$, 
I.~Raniuk$^{42}$, 
N.~Rauschmayr$^{37}$, 
G.~Raven$^{41}$, 
S.~Redford$^{54}$, 
M.M.~Reid$^{47}$, 
A.C.~dos~Reis$^{1}$, 
S.~Ricciardi$^{48}$, 
A.~Richards$^{52}$, 
K.~Rinnert$^{51}$, 
V.~Rives~Molina$^{35}$, 
D.A.~Roa~Romero$^{5}$, 
P.~Robbe$^{7}$, 
D.A.~Roberts$^{57}$, 
E.~Rodrigues$^{53}$, 
P.~Rodriguez~Perez$^{36}$, 
S.~Roiser$^{37}$, 
V.~Romanovsky$^{34}$, 
A.~Romero~Vidal$^{36}$, 
J.~Rouvinet$^{38}$, 
T.~Ruf$^{37}$, 
F.~Ruffini$^{22}$, 
H.~Ruiz$^{35}$, 
P.~Ruiz~Valls$^{35}$, 
G.~Sabatino$^{24,k}$, 
J.J.~Saborido~Silva$^{36}$, 
N.~Sagidova$^{29}$, 
P.~Sail$^{50}$, 
B.~Saitta$^{15,d}$, 
V.~Salustino~Guimaraes$^{2}$, 
B.~Sanmartin~Sedes$^{36}$, 
M.~Sannino$^{19,i}$, 
R.~Santacesaria$^{24}$, 
C.~Santamarina~Rios$^{36}$, 
E.~Santovetti$^{23,k}$, 
M.~Sapunov$^{6}$, 
A.~Sarti$^{18,l}$, 
C.~Satriano$^{24,m}$, 
A.~Satta$^{23}$, 
M.~Savrie$^{16,e}$, 
D.~Savrina$^{30,31}$, 
P.~Schaack$^{52}$, 
M.~Schiller$^{41}$, 
H.~Schindler$^{37}$, 
M.~Schlupp$^{9}$, 
M.~Schmelling$^{10}$, 
B.~Schmidt$^{37}$, 
O.~Schneider$^{38}$, 
A.~Schopper$^{37}$, 
M.-H.~Schune$^{7}$, 
R.~Schwemmer$^{37}$, 
B.~Sciascia$^{18}$, 
A.~Sciubba$^{24}$, 
M.~Seco$^{36}$, 
A.~Semennikov$^{30}$, 
K.~Senderowska$^{26}$, 
I.~Sepp$^{52}$, 
N.~Serra$^{39}$, 
J.~Serrano$^{6}$, 
P.~Seyfert$^{11}$, 
M.~Shapkin$^{34}$, 
I.~Shapoval$^{16,42}$, 
P.~Shatalov$^{30}$, 
Y.~Shcheglov$^{29}$, 
T.~Shears$^{51,37}$, 
L.~Shekhtman$^{33}$, 
O.~Shevchenko$^{42}$, 
V.~Shevchenko$^{30}$, 
A.~Shires$^{52}$, 
R.~Silva~Coutinho$^{47}$, 
M.~Sirendi$^{46}$, 
T.~Skwarnicki$^{58}$, 
N.A.~Smith$^{51}$, 
E.~Smith$^{54,48}$, 
J.~Smith$^{46}$, 
M.~Smith$^{53}$, 
M.D.~Sokoloff$^{56}$, 
F.J.P.~Soler$^{50}$, 
F.~Soomro$^{18}$, 
D.~Souza$^{45}$, 
B.~Souza~De~Paula$^{2}$, 
B.~Spaan$^{9}$, 
A.~Sparkes$^{49}$, 
P.~Spradlin$^{50}$, 
F.~Stagni$^{37}$, 
S.~Stahl$^{11}$, 
O.~Steinkamp$^{39}$, 
S.~Stevenson$^{54}$, 
S.~Stoica$^{28}$, 
S.~Stone$^{58}$, 
B.~Storaci$^{39}$, 
M.~Straticiuc$^{28}$, 
U.~Straumann$^{39}$, 
V.K.~Subbiah$^{37}$, 
L.~Sun$^{56}$, 
S.~Swientek$^{9}$, 
V.~Syropoulos$^{41}$, 
M.~Szczekowski$^{27}$, 
P.~Szczypka$^{38,37}$, 
T.~Szumlak$^{26}$, 
S.~T'Jampens$^{4}$, 
M.~Teklishyn$^{7}$, 
E.~Teodorescu$^{28}$, 
F.~Teubert$^{37}$, 
C.~Thomas$^{54}$, 
E.~Thomas$^{37}$, 
J.~van~Tilburg$^{11}$, 
V.~Tisserand$^{4}$, 
M.~Tobin$^{38}$, 
S.~Tolk$^{41}$, 
D.~Tonelli$^{37}$, 
S.~Topp-Joergensen$^{54}$, 
N.~Torr$^{54}$, 
E.~Tournefier$^{4,52}$, 
S.~Tourneur$^{38}$, 
M.T.~Tran$^{38}$, 
M.~Tresch$^{39}$, 
A.~Tsaregorodtsev$^{6}$, 
P.~Tsopelas$^{40}$, 
N.~Tuning$^{40}$, 
M.~Ubeda~Garcia$^{37}$, 
A.~Ukleja$^{27}$, 
D.~Urner$^{53}$, 
A.~Ustyuzhanin$^{52,p}$, 
U.~Uwer$^{11}$, 
V.~Vagnoni$^{14}$, 
G.~Valenti$^{14}$, 
A.~Vallier$^{7}$, 
M.~Van~Dijk$^{45}$, 
R.~Vazquez~Gomez$^{18}$, 
P.~Vazquez~Regueiro$^{36}$, 
C.~V\'{a}zquez~Sierra$^{36}$, 
S.~Vecchi$^{16}$, 
J.J.~Velthuis$^{45}$, 
M.~Veltri$^{17,g}$, 
G.~Veneziano$^{38}$, 
M.~Vesterinen$^{37}$, 
B.~Viaud$^{7}$, 
D.~Vieira$^{2}$, 
X.~Vilasis-Cardona$^{35,n}$, 
A.~Vollhardt$^{39}$, 
D.~Volyanskyy$^{10}$, 
D.~Voong$^{45}$, 
A.~Vorobyev$^{29}$, 
V.~Vorobyev$^{33}$, 
C.~Vo\ss$^{60}$, 
H.~Voss$^{10}$, 
R.~Waldi$^{60}$, 
C.~Wallace$^{47}$, 
R.~Wallace$^{12}$, 
S.~Wandernoth$^{11}$, 
J.~Wang$^{58}$, 
D.R.~Ward$^{46}$, 
N.K.~Watson$^{44}$, 
A.D.~Webber$^{53}$, 
D.~Websdale$^{52}$, 
M.~Whitehead$^{47}$, 
J.~Wicht$^{37}$, 
J.~Wiechczynski$^{25}$, 
D.~Wiedner$^{11}$, 
L.~Wiggers$^{40}$, 
G.~Wilkinson$^{54}$, 
M.P.~Williams$^{47,48}$, 
M.~Williams$^{55}$, 
F.F.~Wilson$^{48}$, 
J.~Wimberley$^{57}$, 
J.~Wishahi$^{9}$, 
W.~Wislicki$^{27}$, 
M.~Witek$^{25}$, 
S.A.~Wotton$^{46}$, 
S.~Wright$^{46}$, 
S.~Wu$^{3}$, 
K.~Wyllie$^{37}$, 
Y.~Xie$^{49,37}$, 
Z.~Xing$^{58}$, 
Z.~Yang$^{3}$, 
R.~Young$^{49}$, 
X.~Yuan$^{3}$, 
O.~Yushchenko$^{34}$, 
M.~Zangoli$^{14}$, 
M.~Zavertyaev$^{10,a}$, 
F.~Zhang$^{3}$, 
L.~Zhang$^{58}$, 
W.C.~Zhang$^{12}$, 
Y.~Zhang$^{3}$, 
A.~Zhelezov$^{11}$, 
A.~Zhokhov$^{30}$, 
L.~Zhong$^{3}$, 
A.~Zvyagin$^{37}$.\bigskip

{\footnotesize \it
$ ^{1}$Centro Brasileiro de Pesquisas F\'{i}sicas (CBPF), Rio de Janeiro, Brazil\\
$ ^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$ ^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$ ^{4}$LAPP, Universit\'{e} de Savoie, CNRS/IN2P3, Annecy-Le-Vieux, France\\
$ ^{5}$Clermont Universit\'{e}, Universit\'{e} Blaise Pascal, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$ ^{6}$CPPM, Aix-Marseille Universit\'{e}, CNRS/IN2P3, Marseille, France\\
$ ^{7}$LAL, Universit\'{e} Paris-Sud, CNRS/IN2P3, Orsay, France\\
$ ^{8}$LPNHE, Universit\'{e} Pierre et Marie Curie, Universit\'{e} Paris Diderot, CNRS/IN2P3, Paris, France\\
$ ^{9}$Fakult\"{a}t Physik, Technische Universit\"{a}t Dortmund, Dortmund, Germany\\
$ ^{10}$Max-Planck-Institut f\"{u}r Kernphysik (MPIK), Heidelberg, Germany\\
$ ^{11}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany\\
$ ^{12}$School of Physics, University College Dublin, Dublin, Ireland\\
$ ^{13}$Sezione INFN di Bari, Bari, Italy\\
$ ^{14}$Sezione INFN di Bologna, Bologna, Italy\\
$ ^{15}$Sezione INFN di Cagliari, Cagliari, Italy\\
$ ^{16}$Sezione INFN di Ferrara, Ferrara, Italy\\
$ ^{17}$Sezione INFN di Firenze, Firenze, Italy\\
$ ^{18}$Laboratori Nazionali dell'INFN di Frascati, Frascati, Italy\\
$ ^{19}$Sezione INFN di Genova, Genova, Italy\\
$ ^{20}$Sezione INFN di Milano Bicocca, Milano, Italy\\
$ ^{21}$Sezione INFN di Padova, Padova, Italy\\
$ ^{22}$Sezione INFN di Pisa, Pisa, Italy\\
$ ^{23}$Sezione INFN di Roma Tor Vergata, Roma, Italy\\
$ ^{24}$Sezione INFN di Roma La Sapienza, Roma, Italy\\
$ ^{25}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak\'{o}w, Poland\\
$ ^{26}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak\'{o}w, Poland\\
$ ^{27}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$ ^{28}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$ ^{29}$Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$ ^{30}$Institute of Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$ ^{31}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$ ^{32}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAN), Moscow, Russia\\
$ ^{33}$Budker Institute of Nuclear Physics (SB RAS) and Novosibirsk State University, Novosibirsk, Russia\\
$ ^{34}$Institute for High Energy Physics (IHEP), Protvino, Russia\\
$ ^{35}$Universitat de Barcelona, Barcelona, Spain\\
$ ^{36}$Universidad de Santiago de Compostela, Santiago de Compostela, Spain\\
$ ^{37}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$ ^{38}$Ecole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$ ^{39}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$ ^{40}$Nikhef National Institute for Subatomic Physics, Amsterdam, The Netherlands\\
$ ^{41}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, The Netherlands\\
$ ^{42}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$ ^{43}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$ ^{44}$University of Birmingham, Birmingham, United Kingdom\\
$ ^{45}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$ ^{46}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$ ^{47}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$ ^{48}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$ ^{49}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$ ^{50}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$ ^{51}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$ ^{52}$Imperial College London, London, United Kingdom\\
$ ^{53}$School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$ ^{54}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$ ^{55}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$ ^{56}$University of Cincinnati, Cincinnati, OH, United States\\
$ ^{57}$University of Maryland, College Park, MD, United States\\
$ ^{58}$Syracuse University, Syracuse, NY, United States\\
$ ^{59}$Pontif\'{i}cia Universidade Cat\'{o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$ ^{60}$Institut f\"{u}r Physik, Universit\"{a}t Rostock, Rostock, Germany, associated to $^{11}$\\
$ ^{61}$Celal Bayar University, Manisa, Turkey, associated to $^{37}$\\
\bigskip
$ ^{a}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$ ^{b}$Universit\`{a} di Bari, Bari, Italy\\
$ ^{c}$Universit\`{a} di Bologna, Bologna, Italy\\
$ ^{d}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$ ^{e}$Universit\`{a} di Ferrara, Ferrara, Italy\\
$ ^{f}$Universit\`{a} di Firenze, Firenze, Italy\\
$ ^{g}$Universit\`{a} di Urbino, Urbino, Italy\\
$ ^{h}$Universit\`{a} di Modena e Reggio Emilia, Modena, Italy\\
$ ^{i}$Universit\`{a} di Genova, Genova, Italy\\
$ ^{j}$Universit\`{a} di Milano Bicocca, Milano, Italy\\
$ ^{k}$Universit\`{a} di Roma Tor Vergata, Roma, Italy\\
$ ^{l}$Universit\`{a} di Roma La Sapienza, Roma, Italy\\
$ ^{m}$Universit\`{a} della Basilicata, Potenza, Italy\\
$ ^{n}$LIFAELS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$ ^{o}$Hanoi University of Science, Hanoi, Viet Nam\\
$ ^{p}$Institute of Physics and Technology, Moscow, Russia\\
$ ^{q}$Universit\`{a} di Padova, Padova, Italy\\
$ ^{r}$Universit\`{a} di Pisa, Pisa, Italy\\
$ ^{s}$Scuola Normale Superiore, Pisa, Italy\\
}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Authors/LHCb_HD_comma_separated_author_2013-06-18.tex <==
LHCb collaboration:
R. Aaij, 
B. Adeva, 
M. Adinolfi, 
C. Adrover, 
A. Affolder, 
Z. Ajaltouni, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. Anderlini, 
J. Anderson, 
R. Andreassen, 
J.E. Andrews, 
F. Andrianala, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
C. Baesso, 
V. Balagura, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
Th. Bauer, 
A. Bay, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
S. Belogurov, 
K. Belous, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
T. Bird, 
A. Bizzeti, 
P.M. Bj\o rnstad, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
A. Borgia, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
T. Brambach, 
J. van den Brand, 
J. Bressieux, 
D. Brett, 
M. Britsch, 
T. Britton, 
N.H. Brook, 
H. Brown, 
I. Burducea, 
A. Bursche, 
G. Busetto, 
J. Buytaert, 
S. Cadeddu, 
O. Callot, 
M. Calvi, 
M. Calvo Gomez, 
A. Camboni, 
P. Campana, 
D. Campora Perez, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
H. Carranza-Mejia, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
P. Chen, 
N. Chiapolini, 
M. Chrzaszcz, 
K. Ciba, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
C. Coca, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
P. David, 
P.N.Y. David, 
A. Davis, 
I. De Bonis, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
W. De Silva, 
P. De Simone, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
A. Di Canto, 
H. Dijkstra, 
M. Dogaru, 
S. Donleavy, 
F. Dordei, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
F. Dupertuis, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
D. van Eijk, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
A. Falabella, 
C. F\"{a}rber, 
G. Fardell, 
C. Farinelli, 
S. Farry, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
C. Fitzpatrick, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
O. Francisco, 
M. Frank, 
C. Frei, 
M. Frosini, 
S. Furcas, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garofoli, 
P. Garosi, 
J. Garra Tico, 
L. Garrido, 
C. Gaspar, 
R. Gauld, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
V. Gibson, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
P. Gorbounov, 
H. Gordon, 
C. Gotti, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
P. Griffith, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
T. Hampson, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
T. Hartmann, 
J. He, 
T. Head, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
J.A. Hernando Morata, 
E. van Herwijnen, 
M. Hess, 
A. Hicheur, 
E. Hicks, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
P. Hopchev, 
W. Hulsbergen, 
P. Hunt, 
T. Huse, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
V. Iakovenko, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
E. Jans, 
P. Jaton, 
A. Jawahery, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
M. Kaballo, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
I.R. Kenyon, 
T. Ketel, 
A. Keune, 
B. Khanji, 
O. Kochebina, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Korolev, 
A. Kozlinskiy, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
M. Kucharczyk, 
V. Kudryavtsev, 
K. Kurek, 
T. Kvaratskheliya, 
V.N. La Thi, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
R.W. Lambert, 
E. Lanciotti, 
G. Lanfranchi, 
C. Langenbruch, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
S. Leo, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
L. Li Gioi, 
M. Liles, 
R. Lindner, 
C. Linn, 
B. Liu, 
G. Liu, 
S. Lohn, 
I. Longstaff, 
J.H. Lopes, 
N. Lopez-March, 
H. Lu, 
D. Lucchesi, 
J. Luisier, 
H. Luo, 
F. Machefert, 
I.V. Machikhiliyan, 
F. Maciuc, 
O. Maev, 
S. Malde, 
G. Manca, 
G. Mancinelli, 
J. Maratas, 
U. Marconi, 
P. Marino, 
R. M\"{a}rki, 
J. Marks, 
G. Martellotti, 
A. Martens, 
A. Mart\'{i}n S\'{a}nchez, 
M. Martinelli, 
D. Martinez Santos, 
D. Martins Tostes, 
A. Martynov, 
A. Massafferri, 
R. Matev, 
Z. Mathe, 
C. Matteuzzi, 
E. Maurice, 
A. Mazurov, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. McSkelly, 
B. Meadows, 
F. Meier, 
M. Meissner, 
M. Merk, 
D.A. Milanes, 
M.-N. Minard, 
J. Molina Rodriguez, 
S. Monteil, 
D. Moran, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
R. Mountain, 
I. Mous, 
F. Muheim, 
K. M\"{u}ller, 
R. Muresan, 
B. Muryn, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
I. Nasteva, 
M. Needham, 
S. Neubert, 
N. Neufeld, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
M. Nicol, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Nomerotski, 
A. Novoselov, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Oggero, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
M. Orlandea, 
J.M. Otalora Goicochea, 
P. Owen, 
A. Oyanguren, 
B.K. Pal, 
A. Palano, 
T. Palczewski, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
C. Parkes, 
C.J. Parkinson, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
G.N. Patrick, 
C. Patrignani, 
C. Pavel-Nicorescu, 
A. Pazos Alvarez, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
E. Perez Trigo, 
A. P\'{e}rez-Calero Yzquierdo, 
P. Perret, 
M. Perrin-Terrin, 
L. Pescatore, 
E. Pesen, 
K. Petridis, 
A. Petrolini, 
A. Phan, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
S. Playfer, 
M. Plo Casasus, 
F. Polci, 
G. Polok, 
A. Poluektov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
A. Powell, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
J.H. Rademacker, 
B. Rakotomiaramanana, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
S. Redford, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
A. Richards, 
K. Rinnert, 
V. Rives Molina, 
D.A. Roa Romero, 
P. Robbe, 
D.A. Roberts, 
E. Rodrigues, 
P. Rodriguez Perez, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
J. Rouvinet, 
T. Ruf, 
F. Ruffini, 
H. Ruiz, 
P. Ruiz Valls, 
G. Sabatino, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
V. Salustino Guimaraes, 
B. Sanmartin Sedes, 
M. Sannino, 
R. Santacesaria, 
C. Santamarina Rios, 
E. Santovetti, 
M. Sapunov, 
A. Sarti, 
C. Satriano, 
A. Satta, 
M. Savrie, 
D. Savrina, 
P. Schaack, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
M. Seco, 
A. Semennikov, 
K. Senderowska, 
I. Sepp, 
N. Serra, 
J. Serrano, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
P. Shatalov, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
O. Shevchenko, 
V. Shevchenko, 
A. Shires, 
R. Silva Coutinho, 
M. Sirendi, 
T. Skwarnicki, 
N.A. Smith, 
E. Smith, 
J. Smith, 
M. Smith, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
A. Sparkes, 
P. Spradlin, 
F. Stagni, 
S. Stahl, 
O. Steinkamp, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
M. Straticiuc, 
U. Straumann, 
V.K. Subbiah, 
L. Sun, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
P. Szczypka, 
T. Szumlak, 
S. T'Jampens, 
M. Teklishyn, 
E. Teodorescu, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
S. Tolk, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
M.T. Tran, 
M. Tresch, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
M. Ubeda Garcia, 
A. Ukleja, 
D. Urner, 
A. Ustyuzhanin, 
U. Uwer, 
V. Vagnoni, 
G. Valenti, 
A. Vallier, 
M. Van Dijk, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
K. Vervink, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
X. Vilasis-Cardona, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
H. Voss, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
A.D. Webber, 
D. Websdale, 
M. Whitehead, 
J. Wicht, 
J. Wiechczynski, 
D. Wiedner, 
L. Wiggers, 
G. Wilkinson, 
M.P. Williams, 
M. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
S.A. Wotton, 
S. Wright, 
S. Wu, 
K. Wyllie, 
Y. Xie, 
Z. Xing, 
Z. Yang, 
R. Young, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
F. Zhang, 
L. Zhang, 
W.C. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
A. Zvyagin


==> src/0._post.tex <==
\addcontentsline{toc}{section}{References}
\setboolean{inbibliography}{true}
\bibliographystyle{LHCb}
\bibliography{Arxiv-Paper}
%\input{Arxiv-Paper.bbl}



==> src/Paper_titleAbs.tex <==
%\maketitle

\begin{titlepage}

\vspace*{-20mm}
%\vspace*{0mm}

\begin{tabular}{ll}\sffamily
\rule{130mm}{0mm}&\sffamily LHCb-PAPER-2013-036 \\
& \\
& \sffamily 7$^{\textrm{th}}$ October 2013 \\ %\today \\


\end{tabular}
\vspace{5mm}

\begin{center}
\vspace{4mm}
{\bf \sffamily \Huge \input{papertitle}} \\
\vspace{4mm}The LHCb Collaboration

\end{center}

\vspace{15mm}

% --- Abstract -------------------------
\begin{abstract}

\label{Abstract}

\input{paperabstract}

\end{abstract}

% -- body ------------------------------

\end{titlepage}



==> src/fourier_result.tex <==
$\Delta m_s =(17.95 \pm 0.40\,\textrm{(rms)} \pm 0.11\,\textrm{(syst)})$\,ps$^{-1}$
